A Module System for Domain-Specific Languages

Domain-specific languages (DSLs) are routinely created to simplify difficult or specialized programming tasks. They expose useful abstractions and design patterns in the form of language constructs, provide static semantics to eagerly detect misuse of these constructs, and dynamic semantics to completely define how language constructs interact. However, implementing and composing DSLs is a non-trivial task, and there is a lack of tools and techniques. We address this problem by presenting a complete module system over LP for DSL construction, reuse, and composition. LP is already useful for DSL design, because it supports executable language specifications using notations familiar to language designers. We extend LP with a module system that is simple (with a few concepts), succinct (for key DSL specification scenarios), and composable (on the level of languages, compilers, and programs). These design choices reflect our use of LP for industrial DSL design. Our module system has been implemented in the FORMULA language, and was used to build key Windows 8 device drivers via DSLs. Though we present our module system as it actually appears in our FORMULA language, our emphasis is on concepts adaptable to other LP languages.

==> formula2tex1.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{domain}~NonDetFSM~{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\color{formula-comment}{\small\texttt{~~~//~FSM~Syntax}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exISyntaxS}{3}:~~}}{\small\texttt{~~~State~~~~::=~\textcolor{formula-keyword}{new}~(id:~\textcolor{formula-keyword}{Integer}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~~Event~~~~::=~\textcolor{formula-keyword}{new}~(id:~\textcolor{formula-keyword}{String}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~~Trans~~~~::=~\textcolor{formula-keyword}{new}~(src:~State,~ev:~Event,~dst:~State).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exISyntaxE}{6}:~~}}{\small\texttt{~~~Init~~~~~::=~\textcolor{formula-keyword}{new}~(st:~State).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\color{formula-comment}{\small\texttt{~~~//~Reachability~judgment}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exIJudgeS}{8}:~~}}{\small\texttt{~~~Reach~~~~::=~(State).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exIJudgeE}{9}:~~}}{\small\texttt{~~~Reach(s)~:-~Init(s);~Reach(s{\textquotesingle}),~Trans(s{\textquotesingle},~{\_},~s).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{10:~}}{\color{formula-comment}{\small\texttt{~~~//~There~must~be~an~initial~state.}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exIConformsS}{11}:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~Init({\_}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{12:~}}{\color{formula-comment}{\small\texttt{~~~//~Initial~states~must~be~{\textquotedbl}defined{\textquotedbl}.}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exIInitDef}{13}:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~i~{\textbar}~i~\textcolor{formula-keyword}{is}~Init,~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~s~\textcolor{formula-keyword}{is}~State,~s~=~i.st~{\}}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{14:~}}{\color{formula-comment}{\small\texttt{~~~//~Transitions~must~be~over~{\textquotedbl}defined{\textquotedbl}~states~/~events.}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{15:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~t~{\textbar}~t~\textcolor{formula-keyword}{is}~Trans,~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~s~\textcolor{formula-keyword}{is}~State,~s~=~t.src~{\}}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{16:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~t~{\textbar}~t~\textcolor{formula-keyword}{is}~Trans,~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~s~\textcolor{formula-keyword}{is}~State,~s~=~t.dst~{\}}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{exIConformsE}{17}:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~t~{\textbar}~t~\textcolor{formula-keyword}{is}~Trans,~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~s~\textcolor{formula-keyword}{is}~Event,~s~=~t.ev~~{\}}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{18:~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}
\gdef \exISyntaxS {\hyperlink{exISyntaxS}{3}}
\gdef \exISyntaxE {\hyperlink{exISyntaxE}{6}}
\gdef \exIJudgeS {\hyperlink{exIJudgeS}{8}}
\gdef \exIJudgeE {\hyperlink{exIJudgeE}{9}}
\gdef \exIConformsS {\hyperlink{exIConformsS}{11}}
\gdef \exIInitDef {\hyperlink{exIInitDef}{13}}
\gdef \exIConformsE {\hyperlink{exIConformsE}{17}}


==> formula2tex10.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{domain}~Actions}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\color{formula-comment}{\small\texttt{~~~////~Declarations}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~~VarDecl~::=~\textcolor{formula-keyword}{fun}~(id:~\textcolor{formula-keyword}{String}~-{\textgreater}~type:~{\{}~BOOL,~INT~{\}}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~~ActDecl~::=~\textcolor{formula-keyword}{fun}~(id:~\textcolor{formula-keyword}{String}~-{\textgreater}~action:~\textcolor{formula-keyword}{any}~Action).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{6:~~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\color{formula-comment}{\small\texttt{~~~////~Action~language~(expressions)}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{8:~~}}{\small\texttt{~~~BoolOp~::=~{\{}~NOT,~AND,~OR~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{9:~~}}{\small\texttt{~~~IntOp~~::=~{\{}~NEG,~ADD,~SUB,~MUL,~DIV~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{10:~}}{\small\texttt{~~~CmpOp~~::=~{\{}~LT,~LE,~GT,~GE,~EQ,~NEQ~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{11:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{12:~}}{\small\texttt{~~~Var~~~::=~\textcolor{formula-keyword}{new}~(id:~\textcolor{formula-keyword}{String}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{13:~}}{\small\texttt{~~~UnApp~::=~\textcolor{formula-keyword}{new}~(op:~{\{}~NEG,~NOT~{\}},~arg1:~\textcolor{formula-keyword}{any}~Expr).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{14:~}}{\small\texttt{~~~BnApp~::=~\textcolor{formula-keyword}{new}~(op:~{\{}~ADD,~SUB,~MUL,~DIV,~AND,~OR~{\}}~+~CmpOp,}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{15:~}}{\small\texttt{~~~~~~~~~~~~~~~~~~arg1:~\textcolor{formula-keyword}{any}~Expr,~arg2:~\textcolor{formula-keyword}{any}~Expr).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{16:~}}{\small\texttt{~~~Expr~~::=~Var~+~UnApp~+~BnApp~+~\textcolor{formula-keyword}{Boolean}~+~\textcolor{formula-keyword}{Integer}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{17:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{18:~}}{\color{formula-comment}{\small\texttt{~~~////~Action~language~(statements)}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{19:~}}{\small\texttt{~~~Asn~::=~\textcolor{formula-keyword}{new}~(var:~\textcolor{formula-keyword}{String},~expr:~\textcolor{formula-keyword}{any}~Expr).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{20:~}}{\small\texttt{~~~ITE~::=~\textcolor{formula-keyword}{new}~(cond:~\textcolor{formula-keyword}{any}~Expr,~true:~\textcolor{formula-keyword}{any}~Action,~false:~\textcolor{formula-keyword}{any}~Action).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{21:~}}{\small\texttt{~~~Seq~::=~\textcolor{formula-keyword}{new}~(act1:~\textcolor{formula-keyword}{any}~Action,~act2:~\textcolor{formula-keyword}{any}~Action).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{22:~}}{\small\texttt{~~~Action~::=~Asn~+~ITE~+~Seq~+~{\{}~NOP~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{23:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{24:~}}{\color{formula-comment}{\small\texttt{~~~////~Static~typing}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{25:~}}{\small\texttt{~~~Sub~::=~(Action~+~Expr).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{26:~}}{\small\texttt{~~~Sub(e)~~~~~~~~~~~~~~~~~~~~:-~ActDecl({\_},~e);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{27:~}}{\small\texttt{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Sub(UnApp({\_},~e));}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{28:~}}{\small\texttt{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Sub(Asn({\_},~e)).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{29:~}}{\small\texttt{~~~Sub(e),~Sub(e{\textquotesingle})~~~~~~~~~~~:-~Sub(BnApp({\_},~e,~e{\textquotesingle}));}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{30:~}}{\small\texttt{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Sub(Seq(e,~e{\textquotesingle})).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{31:~}}{\small\texttt{~~~Sub(e),~Sub(e{\textquotesingle}),~Sub(e{\textquotesingle}{\textquotesingle})~:-~Sub(ITE(e,~e{\textquotesingle},~e{\textquotesingle}{\textquotesingle})).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{32:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{33:~}}{\small\texttt{~~~TypeJudge~::=~(Action~+~Expr,~{\{}~BOOL,~INT,~ANY~{\}}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{34:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{35:~}}{\small\texttt{~~~TypeJudge(e,~INT)~:-}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{36:~}}{\small\texttt{~~~~~~Sub(e),~e~:~\textcolor{formula-keyword}{Integer};}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{37:~}}{\small\texttt{~~~~~~Sub(e),~e~=~Var(n),~VarDecl(n,~INT);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{38:~}}{\small\texttt{~~~~~~Sub(e),~e~=~UnApp(op,~e{\textquotesingle}),~op~:~IntOp,~TypeJudge(e{\textquotesingle},~INT);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{39:~}}{\small\texttt{~~~~~~Sub(e),~e~=~Asn(n,~e{\textquotesingle}),~VarDecl(n,~INT),~TypeJudge(e{\textquotesingle},~INT);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{40:~}}{\small\texttt{~~~~~~Sub(e),~e~=~BnApp(op,~e{\textquotesingle},~e{\textquotesingle}{\textquotesingle}),~op~:~IntOp,}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{41:~}}{\small\texttt{~~~~~~~~~TypeJudge(e{\textquotesingle},~INT),~TypeJudge(e{\textquotesingle}{\textquotesingle},~INT).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{42:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{43:~}}{\small\texttt{~~~TypeJudge(e,~BOOL)~:-}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{44:~}}{\small\texttt{~~~~~~Sub(e),~e~:~\textcolor{formula-keyword}{Boolean};}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{45:~}}{\small\texttt{~~~~~~Sub(e),~e~=~Var(n),~VarDecl(n,~BOOL);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{46:~}}{\small\texttt{~~~~~~Sub(e),~e~=~UnApp(op,~e{\textquotesingle}),~op~:~BoolOp,~TypeJudge(e{\textquotesingle},~BOOL);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{47:~}}{\small\texttt{~~~~~~Sub(e),~e~=~Asn(n,~e{\textquotesingle}),~VarDecl(n,~BOOL),~TypeJudge(e{\textquotesingle},~BOOL).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{48:~}}{\small\texttt{~~~~~~Sub(e),~e~=~BnApp(op,~e{\textquotesingle},~e{\textquotesingle}{\textquotesingle}),~op~:~BoolOp,}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{49:~}}{\small\texttt{~~~~~~~~~TypeJudge(e{\textquotesingle},~BOOL),~TypeJudge(e{\textquotesingle}{\textquotesingle},~BOOL);}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{50:~}}{\small\texttt{~~~~~~Sub(e),~e~=~BnApp(op,~e{\textquotesingle},~e{\textquotesingle}{\textquotesingle}),~op~:~CmpOp,}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{51:~}}{\small\texttt{~~~~~~~~~TypeJudge(e{\textquotesingle},~t),~TypeJudge(e{\textquotesingle}{\textquotesingle},~t).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{52:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{53:~}}{\small\texttt{~~~TypeJudge(e,~ANY)~:-}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{54:~}}{\small\texttt{~~~~~~Sub(e),~e~=~NOP;}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{55:~}}{\small\texttt{~~~~~~Sub(e),~e~=~Seq(e{\textquotesingle},~e{\textquotesingle}{\textquotesingle}),~TypeJudge(e{\textquotesingle},~{\_}),~TypeJudge(e{\textquotesingle}{\textquotesingle},~{\_});}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{56:~}}{\small\texttt{~~~~~~Sub(e),~e~=~ITE(e{\textquotesingle},~e{\textquotesingle}{\textquotesingle},~e{\textquotesingle}{\textquotesingle}{\textquotesingle}),~TypeJudge(e{\textquotesingle},~BOOL),}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{57:~}}{\small\texttt{~~~~~~~~~TypeJudge(e{\textquotesingle}{\textquotesingle},~{\_}),~TypeJudge(e{\textquotesingle}{\textquotesingle}{\textquotesingle},~{\_}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{58:~}}{\small\texttt{~}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{59:~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~e~{\textbar}~Sub(e),~\textcolor{formula-keyword}{no}~{\{}~t~{\textbar}~TypeJudge(e,~t)~{\}}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{60:~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex2.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{model}~OneStateMach~\textcolor{formula-keyword}{of}~NonDetFSM}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\small\texttt{~~~State(1).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~~Event({\textquotedbl}foo{\textquotedbl}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~~Init(State(1)).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{6:~~}}{\small\texttt{~~~Trans(State(1),~Event({\textquotedbl}foo{\textquotedbl}),}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\small\texttt{~~~~~~~~~State(1)).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{8:~~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex3.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{9:~~}}{\small\texttt{\textcolor{formula-keyword}{model}~TwoStateMach~\textcolor{formula-keyword}{of}~NonDetFSM~{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{10:~}}{\small\texttt{~~~s1~\textcolor{formula-keyword}{is}~State(1).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{11:~}}{\small\texttt{~~~s2~\textcolor{formula-keyword}{is}~State(2).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{12:~}}{\small\texttt{~~~eFoo~\textcolor{formula-keyword}{is}~Event({\textquotedbl}foo{\textquotedbl}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{13:~}}{\small\texttt{~~~Init(s1).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{14:~}}{\small\texttt{~~~Trans(s1,~eFoo,~s2).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{15:~}}{\small\texttt{~~~Trans(s2,~eFoo,~s2).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{16:~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex4.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{17:~}}{\small\texttt{\textcolor{formula-keyword}{model}~BadMach~\textcolor{formula-keyword}{of}~NonDetFSM~{\{}~State(1).~Init(State(100)).~Event({\textquotedbl}Bar{\textquotedbl}).~{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex5.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{domain}~DetFSMWithActions~\textcolor{formula-keyword}{extends}~NonDetFSM,~Actions}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\small\texttt{~~~ActMap~::=~\textcolor{formula-keyword}{fun}~(state:~State~-{\textgreater}~actionName:~\textcolor{formula-keyword}{String}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{count}({\{}~s~{\textbar}~Init(s)~{\}})~=~1.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~Trans(s,~e,~s{\textquotesingle}),~Trans(s,~e,~s{\textquotesingle}{\textquotesingle}),~s{\textquotesingle}~!=~s{\textquotesingle}{\textquotesingle}~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{6:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~s~{\textbar}~s~\textcolor{formula-keyword}{is}~State,~\textcolor{formula-keyword}{no}~Reach(s)~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{conforms}~\textcolor{formula-keyword}{no}~{\{}~a~{\textbar}~ActMap({\_},~a),~\textcolor{formula-keyword}{no}~ActDecl(a,~{\_})~{\}}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{8:~~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex6.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{model}~CntrActions~\textcolor{formula-keyword}{of}~Actions}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\small\texttt{~~VarDecl({\textquotedbl}X{\textquotedbl},~INT).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~ActDecl({\textquotedbl}ZeroX{\textquotedbl},~Asn({\textquotedbl}X{\textquotedbl},~0)).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~ActDecl({\textquotedbl}IncX{\textquotedbl},~Asn({\textquotedbl}X{\textquotedbl},~BnApp(ADD,~Var({\textquotedbl}X{\textquotedbl}),~1))).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{6:~~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\small\texttt{\textcolor{formula-keyword}{model}~CntrMach~\textcolor{formula-keyword}{of}~DetFSMWithActions~\textcolor{formula-keyword}{includes}~TwoStateMach,~CntrActions}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{8:~~}}{\small\texttt{{\{}~ActMap(s1,~{\textquotedbl}ZeroX{\textquotedbl}).~ActMap(s2,~{\textquotedbl}IncX{\textquotedbl}).~{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex7.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{domain}~ParallelFSMs~\textcolor{formula-keyword}{extends}~left::DetFSMWithActions,~right::DetFSMWithActions}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}{\}}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\small\texttt{\textcolor{formula-keyword}{model}~ParallelCntrs~\textcolor{formula-keyword}{of}~ParallelFSMs~\textcolor{formula-keyword}{includes}~left::CntrMach,~right::CntrMach}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{{\{}{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex8.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{transform}~Prune~(in::~NonDetFSM)~\textcolor{formula-keyword}{returns}~(out::~NonDetFSM)}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{ReqConf}{3}:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{requires}~in.\textcolor{formula-keyword}{conforms}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{EnsConf}{4}:~~}}{\small\texttt{~~~\textcolor{formula-keyword}{ensures}~out.\textcolor{formula-keyword}{conforms}.}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{eventCopy}{5}:~~}}{\small\texttt{~~~out.Event(n)~:-~in.Event(n).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{stateCopy}{6}:~~}}{\small\texttt{~~~out.State(x)~:-~in.Reach(State(x)).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{\hypertarget{initCopy}{7}:~~}}{\small\texttt{~~~out.Init(s)~~:-~in.Init(s).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{8:~~}}{\small\texttt{~~~out.Trans(s,~e,~s{\textquotesingle})~:-~in.Trans(s,~e,~s{\textquotesingle}),~in.Reach(s),~in.Reach(s{\textquotesingle}).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{9:~~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}
\gdef \ReqConf {\hyperlink{ReqConf}{3}}
\gdef \EnsConf {\hyperlink{EnsConf}{4}}
\gdef \eventCopy {\hyperlink{eventCopy}{5}}
\gdef \stateCopy {\hyperlink{stateCopy}{6}}
\gdef \initCopy {\hyperlink{initCopy}{7}}


==> formula2tex9.tex <==
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}\vspace{0.5\baselineskip}
 {\tiny\texttt{1:~~}}{\small\texttt{\textcolor{formula-keyword}{transform}~\textcolor{formula-keyword}{system}~PruneAndParallelize~(in1::~NonDetFSM,~in2::~NonDetFSM)}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{2:~~}}{\small\texttt{\textcolor{formula-keyword}{returns}~(out::~ParallelFSMs)}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{3:~~}}{\small\texttt{{\{}}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{4:~~}}{\small\texttt{~~~prune1~=~Prune(in1).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{5:~~}}{\small\texttt{~~~prune2~=~Prune(in2).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{6:~~}}{\small\texttt{~~~out~~~~=~Parallelize(prune1,~prune2).}}
\end{minipage}}\vspace{-3pt}
\fcolorbox{formula-background-gray}{formula-background-gray}{
\begin{minipage}{\codewidthper\textwidth}
 {\tiny\texttt{7:~~}}{\small\texttt{{\}}}}
\end{minipage}}\vspace{-3pt}


==> formula2tex_suffix1.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix10.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix2.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix3.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix4.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix5.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix6.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix7.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix8.tex <==
% this file contains no useful text, but must be present

==> formula2tex_suffix9.tex <==
% this file contains no useful text, but must be present
